Missing bright red giants in the Galactic center: A fingerprint of its once active state?

In the Galactic center nuclear star cluster, bright late-type stars exhibit a flat or even a decreasing surface-density profile, while fainter late-type stars maintain a cusp-like profile. Historically, the lack of red giants in the Galactic center was discovered via the drop in the strength of the CO absorption bandhead by Kris Sellgren et al. (1990), later followed by the stellar number counts based on the high angular resolution near-infrared observations. Several mechanisms were put forward that could have led to the preferential depletion of bright red giants: star-star collisions, tidal stripping, star-accretion disc collisions, or an infall of a massive cluster or a secondary black hole. Here we propose a novel scenario for the bright red-giant depletion based on the collisions between red giants and the nuclear jet, which was likely active in the Galactic center a few million years ago and could have led to the formation of the large-scale $\gamma$-ray Fermi bubbles. The process of the jet-induced ablation of red giants appears to be most efficient within $\sim 0.04\,{\rm pc}$ (S-cluster), while at larger distances it was complemented by star-accretion disc collisions and at smaller scales, tidal stripping operated. These three mechanisms likely operated simultaneously and created an apparent core of late-type stars within $\sim 0.5\,{\rm pc}$.

==> refdef.tex <==
% C:/DOC/WORK/TXT/reference/refdef
% aka
% @article{new, crossref = "real"}

\def\prc{Phys. Rev. C}
\def\pre{Phys. Rev. E}
\def\prd{Phys. Rev. D}
\def\jcap{Journal of Cosmology and Astroparticle Physics}
\def\apss{Astrophysics and Space Science}
\def\mnras{Monthly Notices of the Royal Astronomical Society}
\def\apj{The Astrophysical Journal}
\def\aap{Astronomy and Astrophysics}
\def\actaa{Acta Astronomica}
\def\pasj{Publications of the Astronomical Society of Japan}
\def\apjl{Astrophysical Journal Letters}
\def\pasa{Publications Astronomical Society of Australia}
\def\nat{Nature}
\def\physrep{Physics Reports}
\def\araa{Annual Review of Astronomy and Astrophysics}
\def\apjs{The Astrophysical Journal Supplement}
\def\aapr{The Astronomy and Astrophysics Review}
\def\procspie{Proceedings of the SPIE}


% short
\def\prc{Phys. Rev. C}
\def\pre{Phys. Rev. E}
\def\prd{Phys. Rev. D}
\def\jcap{Journal of Cosmology and Astroparticle Physics}
\def\apss{Astrophysics and Space Science}
\def\mnras{Mon. Not. R. Astron Soc.}
\def\apj{The Astrophysical Journal}
\def\aap{Astron. Astrophys.}
\def\actaa{Acta Astronomica}
\def\pasj{Publications of the Astronomical Society of Japan}
\def\apjl{Astrophysical Journal Letters}
\def\pasa{Publications Astronomical Society of Australia}
\def\nat{Nature}
\def\physrep{Phys. Rep.}
\def\araa{Annu. Rev. Astron. Astrophys.}
\def\apjs{The Astrophysical Journal Supplement}
\def\aapr{The Astronomy and Astrophysics Review}

\def\mdash{---}
